Control VAR: a counterfactual based approach to inference in macroeconomics

A recursive VAR is read as causal whenever the policy is ordered first. I show that this ordering is not sufficient when the policy reacts to the economy it is meant to affect: the impulse response then combines the causal effect with a bias from the common trends that the policy reacts to and a bias specific to the treated unit. I develop the Control VAR (CVAR), which compares the treated unit with untreated controls that share its stochastic trends, and removes the first bias and, under exogeneity with respect to the counterfactual cycle, the second. The method allows repeated, continuous and multiple policies, separates the effect of a single policy change from that of its later values, measures the bias of a VAR without controls through the response of the controls, and bounds the remaining bias. I estimate the weights, derive bootstrap inference, show that the CVAR in changes remains valid when the treated unit has a stochastic trend of its own, test whether the more efficient CVAR in levels is supported, and characterise the bias of weights estimated in changes. I apply the CVAR to the Alaska Permanent Fund Dividend, extended unemployment benefits and California's Low Carbon Fuel Standard.

==> exhibits/fig_california_main_float.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=\textwidth]{fig_california_main.pdf}
\caption{Pass-through of the LCFS cost to the California retail gasoline price}
\label{fig:california_main}
\begin{minipage}{0.95\textwidth}\footnotesize
Note: cumulated response of the California retail price, in cents per gallon, to an increase of 1 cent per gallon in the LCFS cost. Solid line and shaded areas: CVAR in the differenced branch with equal weights on the controls named in each panel, with 68 and 90 percent residual bootstrap bands. Dashed and dotted lines: VAR without controls in the LCFS cost and the change in the California price, with its 90 percent band. Dash-dotted line: full pass-through.
\end{minipage}
\end{figure}


==> exhibits/tab_alaska_adjusted.tex <==
\begin{table}[htbp]
\centering
\caption{Responses adjusted for the common movement left in the cycle\label{tab:ak-adjusted}}
\footnotesize
\begin{tabular}{lcccc}
\toprule
 & \multicolumn{2}{c}{Estimated weights} & \multicolumn{2}{c}{Equal weights} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
Months & CVAR & Adjusted & CVAR & Adjusted \\
\midrule
\multicolumn{5}{l}{Employment-population ratio} \\
12 & $-$0.08 & $-$0.08 & 0.06 & $-$0.07 \\
 & [$-$0.24, 0.10] & [$-$0.23, 0.08] & [$-$0.13, 0.23] & [$-$0.22, 0.09] \\
24 & $-$0.16 & $-$0.15 & 0.07 & $-$0.14 \\
 & [$-$0.42, 0.14] & [$-$0.37, 0.09] & [$-$0.26, 0.35] & [$-$0.38, 0.12] \\
\addlinespace
\multicolumn{5}{l}{Unemployment rate} \\
12 & 0.01 & $-$0.01 & $-$0.10 & $-$0.01 \\
 & [$-$0.18, 0.16] & [$-$0.16, 0.14] & [$-$0.33, 0.14] & [$-$0.17, 0.15] \\
24 & 0.03 & 0.02 & $-$0.15 & 0.01 \\
 & [$-$0.26, 0.27] & [$-$0.22, 0.24] & [$-$0.52, 0.24] & [$-$0.25, 0.27] \\
\addlinespace
\multicolumn{5}{l}{Participation rate} \\
12 & $-$0.15 & $-$0.10 & 0.00 & $-$0.10 \\
 & [$-$0.29, 0.01] & [$-$0.23, 0.02] & [$-$0.15, 0.13] & [$-$0.23, 0.03] \\
24 & $-$0.25$^{*}$ & $-$0.16 & $-$0.02 & $-$0.16 \\
 & [$-$0.45, $-$0.01] & [$-$0.32, 0.00] & [$-$0.22, 0.17] & [$-$0.33, 0.03] \\
\addlinespace
\multicolumn{5}{l}{Payroll employment} \\
12 & 0.42$^{*}$ & 0.67$^{*}$ & 1.17$^{*}$ & 0.68$^{*}$ \\
 & [0.03, 1.00] & [0.22, 1.04] & [0.65, 1.75] & [0.21, 1.04] \\
24 & 0.77$^{*}$ & 1.20$^{*}$ & 2.24$^{*}$ & 1.25$^{*}$ \\
 & [0.10, 1.70] & [0.41, 1.75] & [1.10, 3.28] & [0.43, 1.90] \\
\addlinespace
\multicolumn{5}{l}{Leisure and hospitality} \\
12 & 1.16$^{*}$ & 1.84$^{*}$ & 1.11$^{*}$ & 1.56$^{*}$ \\
 & [0.38, 1.93] & [0.97, 2.73] & [0.48, 1.77] & [0.80, 2.31] \\
24 & 1.71$^{*}$ & 3.17$^{*}$ & 1.63$^{*}$ & 2.62$^{*}$ \\
 & [0.53, 2.76] & [1.51, 4.60] & [0.64, 2.50] & [1.14, 3.81] \\
\addlinespace
\multicolumn{5}{l}{Retail trade} \\
12 & 0.21 & 0.46 & 0.64 & 0.34 \\
 & [$-$0.67, 1.04] & [$-$0.39, 1.20] & [$-$0.34, 1.46] & [$-$0.48, 1.06] \\
24 & 0.37 & 0.86 & 1.08 & 0.65 \\
 & [$-$1.06, 1.66] & [$-$0.52, 1.93] & [$-$0.47, 2.34] & [$-$0.68, 1.70] \\
\bottomrule
\end{tabular}
\par\smallskip\parbox{0.95\textwidth}{\footnotesize Response to a dividend of \$1,000 per person with the six donors, 90 percent bands below the estimates. CVAR: as in Table \ref{tab:ak-main}. Adjusted: response of Alaska relative to the weighted donors in the VAR with both, minus $(1-r)/r$ times the response of the weighted donors, with $r$ the reproduced share in Table \ref{tab:ak-weights} (Proposition \ref{prop:wchanges}), computed in each bootstrap draw with $r$ and the weights held at their estimates. $^{*}$: the 90 percent band excludes zero.}
\end{table}


==> exhibits/tab_alaska_bounds.tex <==
\begin{table}[htbp]
\centering
\caption{Sensitivity to a bias specific to Alaska\label{tab:ak-bounds}}
\footnotesize
\begin{tabular}{lcccccc}
\toprule
Months & CVAR & Weighted & $\lambda=0$ & $\lambda=0.5$ & $\lambda=1$ & $\lambda$ reaching \\
 & & controls & & & & zero \\
\midrule
\multicolumn{7}{l}{Employment-population ratio} \\
12 & $-$0.09 & $-$0.14 & [$-$0.25, 0.07] & [$-$0.31, 0.15] & [$-$0.40, 0.25] & 0.00 \\
24 & $-$0.16 & $-$0.24 & [$-$0.39, 0.09] & [$-$0.52, 0.22] & [$-$0.68, 0.39] & 0.00 \\
\addlinespace
\multicolumn{7}{l}{Participation rate} \\
12 & $-$0.15 & $-$0.06 & [$-$0.29, $-$0.03] & [$-$0.33, 0.00] & [$-$0.36, 0.03] & 0.50 \\
24 & $-$0.26 & $-$0.13 & [$-$0.45, $-$0.07] & [$-$0.53, $-$0.02] & [$-$0.61, 0.04] & 0.70 \\
\addlinespace
\multicolumn{7}{l}{Payroll employment} \\
12 & 0.51 & $-$0.25 & [0.10, 0.87] & [$-$0.04, 1.00] & [$-$0.18, 1.14] & 0.36 \\
24 & 0.88 & $-$0.51 & [0.21, 1.39] & [$-$0.06, 1.67] & [$-$0.35, 1.96] & 0.40 \\
\addlinespace
\multicolumn{7}{l}{Leisure and hospitality} \\
12 & 1.13 & $-$0.96 & [0.52, 1.76] & [0.05, 2.40] & [$-$0.62, 3.11] & 0.54 \\
24 & 1.80 & $-$1.86 & [0.81, 2.66] & [0.00, 3.97] & [$-$1.23, 5.33] & 0.51 \\
\bottomrule
\end{tabular}
\par\smallskip\parbox{0.95\textwidth}{\footnotesize From the VAR with Alaska and the weighted controls (Proposition \ref{prop:placebo}), 90 percent bands for the bounds of Proposition \ref{prop:bounds}, with the bias specific to Alaska at most $\lambda$ times the bias from the common trends, measured by the response of the weighted controls. Weights held at their estimates. Last column: smallest $\lambda$ at which the band contains zero.}
\end{table}


==> exhibits/tab_alaska_pools.tex <==
\begin{table}[htbp]
\centering
\caption{Alaska: larger donor pools\label{tab:ak-pools}}
\footnotesize
\begin{tabular}{lccc}
\toprule
 & Six donors & West & All states \\
\midrule
\multicolumn{4}{l}{Employment-population ratio} \\
Reproduced & 0.98 & 1.02 & 1.14 \\
12 months & $-$0.08 & $-$0.09 & $-$0.05 \\
 & [$-$0.24, 0.10] & [$-$0.25, 0.09] & [$-$0.21, 0.14] \\
24 months & $-$0.16 & $-$0.18 & $-$0.10 \\
 & [$-$0.42, 0.14] & [$-$0.44, 0.12] & [$-$0.37, 0.21] \\
\addlinespace
\multicolumn{4}{l}{Unemployment rate} \\
Reproduced & 0.86 & 0.96 & 1.12 \\
12 months & 0.01 & $-$0.00 & $-$0.01 \\
 & [$-$0.18, 0.16] & [$-$0.20, 0.16] & [$-$0.20, 0.14] \\
24 months & 0.03 & 0.01 & $-$0.02 \\
 & [$-$0.26, 0.27] & [$-$0.29, 0.26] & [$-$0.31, 0.23] \\
\addlinespace
\multicolumn{4}{l}{Participation rate} \\
Reproduced & 0.57 & 1.01 & 1.33 \\
12 months & $-$0.15 & $-$0.14 & $-$0.10 \\
 & [$-$0.29, 0.01] & [$-$0.28, 0.02] & [$-$0.22, 0.07] \\
24 months & $-$0.25$^{*}$ & $-$0.23 & $-$0.17 \\
 & [$-$0.45, $-$0.01] & [$-$0.42, 0.01] & [$-$0.34, 0.08] \\
\addlinespace
\multicolumn{4}{l}{Payroll employment} \\
Reproduced & 0.61 & 0.86 & 1.34 \\
12 months & 0.42$^{*}$ & 0.51$^{*}$ & 0.84$^{*}$ \\
 & [0.03, 1.00] & [0.17, 1.07] & [0.44, 1.46] \\
24 months & 0.77$^{*}$ & 0.92$^{*}$ & 1.46$^{*}$ \\
 & [0.10, 1.70] & [0.30, 1.87] & [0.74, 2.48] \\
\addlinespace
\multicolumn{4}{l}{Leisure and hospitality} \\
Reproduced & 0.58 & 0.81 & 1.41 \\
12 months & 1.16$^{*}$ & 1.55$^{*}$ & 1.40$^{*}$ \\
 & [0.38, 1.93] & [0.72, 2.64] & [0.72, 2.49] \\
24 months & 1.71$^{*}$ & 2.40$^{*}$ & 2.13$^{*}$ \\
 & [0.53, 2.76] & [1.07, 4.10] & [1.02, 3.90] \\
\addlinespace
\multicolumn{4}{l}{Retail trade} \\
Reproduced & 0.63 & 0.95 & 1.24 \\
12 months & 0.21 & 0.56 & 0.52 \\
 & [$-$0.67, 1.04] & [$-$0.31, 1.42] & [$-$0.39, 1.36] \\
24 months & 0.37 & 0.92 & 0.82 \\
 & [$-$1.06, 1.66] & [$-$0.51, 2.23] & [$-$0.50, 2.04] \\
\bottomrule
\end{tabular}
\par\smallskip\parbox{0.95\textwidth}{\footnotesize CVAR of Table \ref{tab:ak-main} with weights estimated in changes from the six donors of the main specification, from the 12 other states of the Census West region, and from all 50 other states and the District of Columbia, with 90 percent bands below the estimates. Reproduced: share of the main common movement of Alaska reproduced by the weighted donors, as in Table \ref{tab:ak-weights}. $^{*}$: the 90 percent band excludes zero.}
\end{table}


==> exhibits/tab_alaska_samples.tex <==
\begin{table}[htbp]
\centering
\caption{Alaska: samples ending before the legislated dividends and before 2008\label{tab:ak-samples}}
\footnotesize
\begin{tabular}{lccc}
\toprule
Months & To 2019 & To 2015 & To 2007 \\
\midrule
\multicolumn{4}{l}{Employment-population ratio} \\
12 & $-$0.08 & $-$0.08 & $-$0.10 \\
 & [$-$0.24, 0.10] & [$-$0.26, 0.09] & [$-$0.36, 0.14] \\
24 & $-$0.16 & $-$0.16 & $-$0.22 \\
 & [$-$0.42, 0.14] & [$-$0.44, 0.12] & [$-$0.61, 0.17] \\
\addlinespace
\multicolumn{4}{l}{Unemployment rate} \\
12 & 0.01 & $-$0.00 & $-$0.02 \\
 & [$-$0.18, 0.16] & [$-$0.19, 0.15] & [$-$0.28, 0.20] \\
24 & 0.03 & 0.01 & 0.01 \\
 & [$-$0.26, 0.27] & [$-$0.29, 0.26] & [$-$0.39, 0.36] \\
\addlinespace
\multicolumn{4}{l}{Participation rate} \\
12 & $-$0.15 & $-$0.17$^{*}$ & $-$0.22 \\
 & [$-$0.29, 0.01] & [$-$0.31, $-$0.01] & [$-$0.42, 0.01] \\
24 & $-$0.25$^{*}$ & $-$0.27$^{*}$ & $-$0.36$^{*}$ \\
 & [$-$0.45, $-$0.01] & [$-$0.47, $-$0.03] & [$-$0.64, $-$0.01] \\
\addlinespace
\multicolumn{4}{l}{Payroll employment} \\
12 & 0.42$^{*}$ & 0.41$^{*}$ & 0.71 \\
 & [0.03, 1.00] & [0.01, 1.01] & [$-$0.06, 1.80] \\
24 & 0.77$^{*}$ & 0.66$^{*}$ & 1.23 \\
 & [0.10, 1.70] & [0.06, 1.58] & [$-$0.13, 3.00] \\
\addlinespace
\multicolumn{4}{l}{Leisure and hospitality} \\
12 & 1.16$^{*}$ & 1.39$^{*}$ & 1.67 \\
 & [0.38, 1.93] & [0.41, 2.43] & [$-$0.38, 3.51] \\
24 & 1.71$^{*}$ & 2.10$^{*}$ & 2.92 \\
 & [0.53, 2.76] & [0.56, 3.48] & [$-$0.55, 5.36] \\
\addlinespace
\multicolumn{4}{l}{Retail trade} \\
12 & 0.21 & $-$0.02 & $-$0.51 \\
 & [$-$0.67, 1.04] & [$-$0.91, 0.82] & [$-$2.13, 2.26] \\
24 & 0.37 & $-$0.08 & $-$0.45 \\
 & [$-$1.06, 1.66] & [$-$1.45, 1.26] & [$-$3.15, 3.94] \\
\bottomrule
\end{tabular}
\par\smallskip\parbox{0.95\textwidth}{\footnotesize CVAR of Table \ref{tab:ak-main} estimated on samples ending in December 2019 (main), December 2015 (before the legislature set the amounts) and December 2007 (before the 2008 dividend, the energy rebate and the recession), with 90 percent bands below the estimates. Rates from January 1976, payroll series from January 1990. Weights re-estimated in each sample. $^{*}$: the 90 percent band excludes zero.}
\end{table}


==> exhibits/tab_alaska_seasonal.tex <==
\begin{table}[htbp]
\centering
\caption{Alaska: treatment of seasonality\label{tab:ak-seasonal}}
\footnotesize
\begin{tabular}{lccccc}
\toprule
Series & Sum of & \multicolumn{4}{c}{Months} \\
\cmidrule(lr){3-6}
 & weights & 1 & 3 & 12 & 24 \\
\midrule
\multicolumn{6}{l}{Employment-population ratio} \\
Adjusted & 0.57 & 0.01 & $-$0.00 & $-$0.08 & $-$0.16 \\
Adjusted, month effects & 0.57 & 0.02 & 0.00 & $-$0.09 & $-$0.17 \\
Unadjusted, month effects & 1.20 & 0.27$^{*}$ & 0.22$^{*}$ & 0.40$^{*}$ & 0.53$^{*}$ \\
Unadjusted, month effects $\times$ trend & 0.94 & 0.24$^{*}$ & 0.19$^{*}$ & 0.35$^{*}$ & 0.47 \\
Unadjusted, month effects by decade & 0.92 & 0.27$^{*}$ & 0.19 & 0.31 & 0.35 \\
\addlinespace
\multicolumn{6}{l}{Unemployment rate} \\
Adjusted & 0.49 & $-$0.01 & $-$0.01 & 0.01 & 0.03 \\
Adjusted, month effects & 0.49 & $-$0.02 & $-$0.03 & $-$0.00 & 0.02 \\
Unadjusted, month effects & 0.98 & $-$0.16$^{*}$ & $-$0.21$^{*}$ & $-$0.15 & $-$0.21 \\
Unadjusted, month effects $\times$ trend & 0.93 & $-$0.13$^{*}$ & $-$0.17$^{*}$ & $-$0.09 & $-$0.12 \\
Unadjusted, month effects by decade & 0.96 & $-$0.10$^{*}$ & $-$0.14$^{*}$ & $-$0.05 & $-$0.07 \\
\addlinespace
\multicolumn{6}{l}{Participation rate} \\
Adjusted & 0.40 & 0.00 & $-$0.02 & $-$0.15$^{*}$ & $-$0.25$^{*}$ \\
Adjusted, month effects & 0.41 & 0.01 & $-$0.02 & $-$0.18$^{*}$ & $-$0.28$^{*}$ \\
Unadjusted, month effects & 1.12 & 0.14 & 0.04 & 0.17 & 0.14 \\
Unadjusted, month effects $\times$ trend & 0.92 & 0.15$^{*}$ & 0.06 & 0.15 & 0.14 \\
Unadjusted, month effects by decade & 0.90 & 0.18$^{*}$ & 0.03 & 0.09 & 0.07 \\
\addlinespace
\multicolumn{6}{l}{Payroll employment} \\
Adjusted & 0.30 & $-$0.02 & 0.05 & 0.42$^{*}$ & 0.77$^{*}$ \\
Adjusted, month effects & 0.27 & $-$0.03 & 0.07 & 0.44 & 0.80$^{*}$ \\
Unadjusted, month effects & 0.33 & 0.02 & 0.43$^{*}$ & $-$0.18 & $-$0.22 \\
Unadjusted, month effects $\times$ trend & 0.30 & 0.04 & 0.33 & 0.21 & 0.49 \\
Unadjusted, month effects by decade & 0.46 & 0.13 & 0.46$^{*}$ & 0.27 & 0.44 \\
\addlinespace
\multicolumn{6}{l}{Leisure and hospitality} \\
Adjusted & 0.90 & $-$0.03 & 0.26 & 1.16$^{*}$ & 1.71$^{*}$ \\
Adjusted, month effects & 0.88 & 0.38 & 0.57$^{*}$ & 1.32$^{*}$ & 1.75$^{*}$ \\
Unadjusted, month effects & 0.65 & 0.65$^{*}$ & 0.50 & 0.65 & 1.05 \\
Unadjusted, month effects $\times$ trend & 0.62 & 0.45 & 0.54 & 0.84$^{*}$ & 1.26$^{*}$ \\
Unadjusted, month effects by decade & 0.61 & 0.46 & 0.44 & 0.93 & 1.12 \\
\addlinespace
\multicolumn{6}{l}{Retail trade} \\
Adjusted & 0.52 & 0.01 & 0.02 & 0.21 & 0.37 \\
Adjusted, month effects & 0.52 & 0.08 & 0.16 & 0.32 & 0.40 \\
Unadjusted, month effects & 0.77 & 0.20 & $-$0.00 & 0.77 & 1.07 \\
Unadjusted, month effects $\times$ trend & 0.43 & $-$0.03 & $-$0.10 & $-$0.12 & $-$0.49 \\
Unadjusted, month effects by decade & 0.49 & $-$0.01 & $-$0.25 & $-$0.39 & $-$0.85 \\
\bottomrule
\end{tabular}
\par\smallskip\parbox{0.95\textwidth}{\footnotesize CVAR of Table \ref{tab:ak-main}, January 1976 (payroll series January 1990) to December 2019, with the seasonally adjusted series (main), the adjusted series with month effects, and the unadjusted series with month effects, with month effects interacted with a linear trend, and with month effects by decade, in the weights regression and in the VAR. Weights re-estimated in each version and held at their estimates in the residual bootstrap. $^{*}$: the 90 percent band excludes zero.}
\end{table}


==> exhibits/tab_california_lp.tex <==
\begin{table}[htbp]
\centering
\caption{Pass-through of the LCFS cost: local projections on the cycle}
\label{tab:california_lp}
\small
\begin{tabular}{lcccc}
\toprule
 & Lags & Impact & 1 month & 12 months \\
\midrule
\multicolumn{5}{l}{Local projections on the cycle} \\
\midrule
Gulf Coast (PADD 3), local projection, linear & 2 & 1.06 & 1.67 & 0.70 \\
\footnotesize  &  & [-0.18, 2.31] & [-0.24, 3.58] & [-2.04, 3.45] \\[2pt]
Gulf Coast (PADD 3), local projection, increases & 2 & 0.14 & 1.02 & -0.21 \\
\footnotesize  &  & [-1.21, 1.49] & [-1.55, 3.59] & [-3.73, 3.30] \\[2pt]
Gulf Coast (PADD 3), local projection, decreases & 2 & 2.48 & 2.67 & 2.01 \\
\footnotesize  &  & [-0.14, 5.10] & [-1.58, 6.91] & [-4.19, 8.20] \\[2pt]
Gulf Coast (PADD 3), local projection, high credit price & 2 & 2.93 & 1.44 & 3.31 \\
\footnotesize  &  & [-0.04, 5.90] & [-3.33, 6.21] & [-2.00, 8.62] \\[2pt]
Gulf Coast (PADD 3), local projection, low credit price & 2 & 0.11 & 1.79$^{*}$ & -0.86 \\
\footnotesize  &  & [-0.98, 1.19] & [0.26, 3.32] & [-2.31, 0.59] \\[2pt]
PADDs 1 to 4, local projection, linear & 2 & 0.77 & 1.75 & 1.07 \\
\footnotesize  &  & [-0.48, 2.02] & [-0.02, 3.53] & [-1.41, 3.55] \\[2pt]
PADDs 1 to 4, local projection, increases & 2 & -0.23 & 1.16 & 0.40 \\
\footnotesize  &  & [-1.44, 0.98] & [-1.17, 3.48] & [-2.75, 3.55] \\[2pt]
PADDs 1 to 4, local projection, decreases & 2 & 2.29 & 2.66 & 2.02 \\
\footnotesize  &  & [-0.54, 5.12] & [-1.30, 6.62] & [-3.86, 7.89] \\[2pt]
PADDs 1 to 4, local projection, high credit price & 2 & 2.41 & 1.52 & 3.31 \\
\footnotesize  &  & [-0.86, 5.68] & [-3.01, 6.05] & [-1.48, 8.10] \\[2pt]
PADDs 1 to 4, local projection, low credit price & 2 & -0.08 & 1.87$^{*}$ & -0.28 \\
\footnotesize  &  & [-1.02, 0.86] & [0.54, 3.21] & [-1.67, 1.12] \\[2pt]
\bottomrule
\end{tabular}
\begin{minipage}{0.95\textwidth}\footnotesize
Note: cumulated response of the California retail price, in cents per gallon, to an increase of 1 cent per gallon in the LCFS cost, from local projections on the CVAR cycle with equal weights on the controls. Policy: the cost per gallon implied by the CARB formula before May 2024 and the cost reported by refiners to the California Energy Commission from then on, in monthly changes. Local projections: regression of the change in the cycle between $t-1$ and $t+h$ on the change in the cost (split into increases and decreases, or interacted with a credit price above or below the sample median at $t-1$), two lags of the changes in the cycle and in the cost, and a constant. 90 percent Newey-West bands in brackets; $^{*}$ the 90 percent band excludes zero.
\end{minipage}
\end{table}


==> exhibits/tab_california_main.tex <==
\begin{table}[htbp]
\centering
\caption{Pass-through of the LCFS cost to the California retail gasoline price\label{tab:california_main}}
\small
\begin{tabular}{lcccc}
\toprule
Controls & Lags & Impact & 1 month & Width ratio \\
\midrule
Gulf Coast (PADD 3) & 4/4 & 0.99$^{\dagger}$ & 1.55$^{\dagger}$ & 0.56 \\
\footnotesize  &  & [-0.21, 2.47] & [-0.42, 3.75] &  \\[2pt]
PADDs 1 to 4 & 4/4 & 0.65 & 1.59$^{\dagger}$ & 0.53 \\
\footnotesize  &  & [-0.46, 1.93] & [-0.28, 3.70] &  \\[2pt]
Texas and Florida & 4/4 & 1.11$^{\dagger}$ & 1.68$^{\dagger}$ & 0.60 \\
\footnotesize  &  & [-0.19, 2.67] & [-0.51, 4.02] &  \\[2pt]
\bottomrule
\end{tabular}
\begin{minipage}{0.95\textwidth}\footnotesize
Note: cumulated response of the California retail price, in cents per gallon, to an increase of 1 cent per gallon in the LCFS cost, from the CVAR in the differenced branch with equal weights on the controls. Policy: the cost per gallon implied by the CARB formula before May 2024 and the cost reported by refiners to the California Energy Commission from then on, in monthly changes, unless stated otherwise. Lags: CVAR / VAR without controls. 90 percent residual bootstrap bands in brackets; $^{\dagger}$ the 68 percent band excludes zero; $^{*}$ the 90 percent band excludes zero. Width ratio: width of the CVAR band over that of the VAR without controls, at one month. The full paths are in Figure \ref{fig:california_main}, and robustness checks in Tables \ref{tab:california_robust}, \ref{tab:california_appendix}, \ref{tab:california_measures} and \ref{tab:california_lp}.
\end{minipage}
\end{table}


==> exhibits/tab_california_measures.tex <==
\begin{table}[htbp]
\centering
\caption{Pass-through of the LCFS cost: policy measures and the 2014 to 2019 sample}
\label{tab:california_measures}
\small
\begin{tabular}{lccccc}
\toprule
 & Lags & Impact & 1 month & 12 months & Width ratio \\
\midrule
\multicolumn{6}{l}{Policy measure} \\
\midrule
Gulf Coast (PADD 3), spliced, January dummy & 2/2 & 1.42$^{\dagger}$ & 1.90$^{\dagger}$ & 1.06 & 0.56 \\
\footnotesize  &  & [-0.54, 3.46] & [-0.66, 4.38] & [-1.21, 3.39] &  \\[2pt]
Gulf Coast (PADD 3), CARB formula only & 12/10 & 2.75$^{*}$ & 2.24$^{\dagger}$ & 1.65 & 0.38 \\
\footnotesize  &  & [0.15, 5.17] & [-1.19, 5.88] & [-2.30, 6.69] &  \\[2pt]
Gulf Coast (PADD 3), constant factor & 2/2 & 1.54$^{*}$ & 1.08 & 0.66 & 0.50 \\
\footnotesize  &  & [0.10, 3.02] & [-1.09, 3.02] & [-1.75, 2.92] &  \\[2pt]
PADDs 1 to 4, spliced, January dummy & 2/2 & 1.04 & 1.83$^{\dagger}$ & 1.12 & 0.55 \\
\footnotesize  &  & [-0.74, 3.09] & [-0.48, 4.16] & [-1.10, 3.46] &  \\[2pt]
PADDs 1 to 4, CARB formula only & 12/10 & 1.65$^{\dagger}$ & 2.22$^{\dagger}$ & 1.60 & 0.37 \\
\footnotesize  &  & [-0.74, 4.06] & [-1.26, 5.46] & [-2.22, 6.40] &  \\[2pt]
PADDs 1 to 4, constant factor & 2/2 & 1.28$^{\dagger}$ & 1.10 & 0.62 & 0.49 \\
\footnotesize  &  & [-0.18, 2.93] & [-0.96, 2.99] & [-1.69, 2.90] &  \\[2pt]
\midrule
\multicolumn{6}{l}{Sample 2014 to 2019} \\
\midrule
Gulf Coast (PADD 3), 2014 to 2019 & 1/1 & -0.62 & -1.94 & -1.90 & 0.68 \\
\footnotesize  &  & [-3.32, 2.22] & [-6.73, 3.37] & [-6.62, 3.17] &  \\[2pt]
Gulf Coast (PADD 3), 2014 to 2019 & 2/2 & -0.36 & -1.31 & -3.67$^{\dagger}$ & 0.56 \\
\footnotesize  &  & [-3.19, 2.61] & [-5.80, 3.47] & [-8.33, 1.05] &  \\[2pt]
PADDs 1 to 4, 2014 to 2019$^{a}$ & 1/1 & -1.47 & 0.02 & 0.01 & 0.07 \\
\footnotesize  &  & [-5.15, 1.49] & [-5.77, 4.25] & [-0.56, 0.47] &  \\[2pt]
PADDs 1 to 4, 2014 to 2019$^{a}$ & 2/2 & -1.60 & -0.05 & -0.11 & 0.06 \\
\footnotesize  &  & [-5.28, 1.95] & [-5.30, 4.32] & [-0.76, 0.24] &  \\[2pt]
\bottomrule
\end{tabular}
\begin{minipage}{0.95\textwidth}\footnotesize
Note: cumulated response of the California retail price, in cents per gallon, to an increase of 1 cent per gallon in the LCFS cost, from the CVAR in the differenced branch with equal weights on the controls. Policy: the cost per gallon implied by the CARB formula before May 2024 and the cost reported by refiners to the California Energy Commission from then on, in monthly changes, unless stated otherwise. Lags: CVAR / VAR without controls. 90 percent residual bootstrap bands in brackets; $^{\dagger}$ the 68 percent band excludes zero; $^{*}$ the 90 percent band excludes zero. Width ratio: width of the CVAR band over that of the VAR without controls, at 12 months. In 2014 to 2019 the cost per gallon implied by the CARB formula is small, so the policy varies little. $^{a}$ The design test rejects in this sample and the CVAR is in levels with estimated weights, where the response of the stationary cycle to a permanent change in the cost returns to zero by construction.
\end{minipage}
\end{table}


==> exhibits/tab_california_robust.tex <==
\begin{table}[htbp]
\centering
\caption{Pass-through of the LCFS cost: samples and controls}
\label{tab:california_robust}
\small
\begin{tabular}{lccccc}
\toprule
 & Lags & Impact & 1 month & 12 months & Width ratio \\
\midrule
\multicolumn{6}{l}{Main specification} \\
\midrule
Gulf Coast (PADD 3) & 4/4 & 0.99$^{\dagger}$ & 1.55$^{\dagger}$ & 0.88 & 0.43 \\
\footnotesize  &  & [-0.21, 2.47] & [-0.42, 3.75] & [-1.08, 3.19] &  \\[2pt]
PADDs 1 to 4 & 4/4 & 0.65 & 1.59$^{\dagger}$ & 0.87 & 0.39 \\
\footnotesize  &  & [-0.46, 1.93] & [-0.28, 3.70] & [-0.97, 2.92] &  \\[2pt]
Texas and Florida & 4/4 & 1.11$^{\dagger}$ & 1.68$^{\dagger}$ & 1.03 & 0.46 \\
\footnotesize  &  & [-0.19, 2.67] & [-0.51, 4.02] & [-1.03, 3.48] &  \\[2pt]
\midrule
\multicolumn{6}{l}{Samples} \\
\midrule
Gulf Coast (PADD 3), 2017 onward & 3/3 & 1.30$^{*}$ & 1.62$^{\dagger}$ & 1.45$^{\dagger}$ & 0.41 \\
\footnotesize  &  & [0.15, 2.82] & [-0.53, 3.98] & [-0.73, 3.81] &  \\[2pt]
Gulf Coast (PADD 3), 2020 onward & 2/2 & 1.78$^{*}$ & 2.15$^{\dagger}$ & 1.38$^{\dagger}$ & 0.44 \\
\footnotesize  &  & [0.39, 3.39] & [-0.18, 4.54] & [-0.54, 3.48] &  \\[2pt]
Gulf Coast (PADD 3), 2014 to 2024 & 12/12 & 2.22$^{\dagger}$ & 1.57 & 1.72 & 0.45 \\
\footnotesize  &  & [-0.84, 5.41] & [-2.42, 5.96] & [-2.85, 8.15] &  \\[2pt]
Gulf Coast (PADD 3), 2020 to 2022 dummied out & 2/2 & 0.68 & 1.84$^{\dagger}$ & 1.53$^{\dagger}$ & 0.66 \\
\footnotesize  &  & [-0.95, 2.05] & [-0.92, 4.25] & [-1.12, 3.84] &  \\[2pt]
PADDs 1 to 4, 2017 onward & 4/3 & 1.02$^{\dagger}$ & 1.56$^{\dagger}$ & 1.31$^{\dagger}$ & 0.32 \\
\footnotesize  &  & [-0.10, 2.39] & [-0.24, 3.63] & [-0.35, 3.21] &  \\[2pt]
PADDs 1 to 4, 2020 onward & 2/2 & 1.49$^{*}$ & 2.21$^{\dagger}$ & 1.44$^{\dagger}$ & 0.45 \\
\footnotesize  &  & [0.19, 3.11] & [-0.03, 4.39] & [-0.47, 3.60] &  \\[2pt]
PADDs 1 to 4, 2014 to 2024 & 12/12 & 1.09 & 1.15 & 1.53 & 0.43 \\
\footnotesize  &  & [-1.81, 4.24] & [-2.79, 5.39] & [-2.87, 7.60] &  \\[2pt]
PADDs 1 to 4, 2020 to 2022 dummied out & 2/2 & 0.30 & 1.70$^{\dagger}$ & 1.36 & 0.65 \\
\footnotesize  &  & [-1.34, 1.66] & [-0.88, 3.79] & [-1.28, 3.61] &  \\[2pt]
\midrule
\multicolumn{6}{l}{Leaving one PADD out} \\
\midrule
PADDs 1 to 4 without East Coast & 4/4 & 0.55 & 1.59$^{\dagger}$ & 0.81 & 0.40 \\
\footnotesize  &  & [-0.50, 1.75] & [-0.18, 3.69] & [-1.08, 2.83] &  \\[2pt]
PADDs 1 to 4 without Midwest & 4/4 & 0.60 & 1.47$^{\dagger}$ & 0.76 & 0.41 \\
\footnotesize  &  & [-0.49, 1.92] & [-0.43, 3.58] & [-1.19, 2.84] &  \\[2pt]
PADDs 1 to 4 without Gulf Coast & 4/4 & 0.53 & 1.58$^{\dagger}$ & 0.86 & 0.39 \\
\footnotesize  &  & [-0.62, 1.82] & [-0.31, 3.71] & [-0.99, 2.88] &  \\[2pt]
PADDs 1 to 4 without Rocky Mountain & 4/4 & 0.91$^{\dagger}$ & 1.68$^{\dagger}$ & 1.02 & 0.41 \\
\footnotesize  &  & [-0.30, 2.41] & [-0.32, 3.91] & [-0.87, 3.19] &  \\[2pt]
\bottomrule
\end{tabular}
\begin{minipage}{0.95\textwidth}\footnotesize
Note: cumulated response of the California retail price, in cents per gallon, to an increase of 1 cent per gallon in the LCFS cost, from the CVAR in the differenced branch with equal weights on the controls. Policy: the cost per gallon implied by the CARB formula before May 2024 and the cost reported by refiners to the California Energy Commission from then on, in monthly changes, unless stated otherwise. Lags: CVAR / VAR without controls. 90 percent residual bootstrap bands in brackets; $^{\dagger}$ the 68 percent band excludes zero; $^{*}$ the 90 percent band excludes zero. Width ratio: width of the CVAR band over that of the VAR without controls, at 12 months.
\end{minipage}
\end{table}


==> exhibits/tab_eb_average.tex <==
\begin{table}[htbp]
\centering
\caption{Response of the unemployment rate to ten additional weeks of EB, average across states\label{tab:eb-avg}}
\small
\begin{tabular}{cccccc}
\toprule
Months & CVAR & VAR without controls & Width ratio & Weighted controls & Impulse causal effect \\
\midrule
0 & $-$0.00 & $-$0.03 & 0.86 & $-$0.01 & $-$0.00 \\
\footnotesize & [$-$0.02, 0.01] & [$-$0.05, $-$0.01] & & [$-$0.03, 0.00] & [$-$0.02, 0.01] \\[2pt]
6 & 0.03 & $-$0.23 & 0.68 & $-$0.24 & 0.00 \\
\footnotesize & [$-$0.03, 0.11] & [$-$0.32, $-$0.11] & & [$-$0.34, $-$0.13] & [$-$0.01, 0.02] \\[2pt]
12 & 0.05 & $-$0.33 & 0.69 & $-$0.37 & $-$0.00 \\
\footnotesize & [$-$0.06, 0.17] & [$-$0.47, $-$0.13] & & [$-$0.51, $-$0.17] & [$-$0.02, 0.01] \\[2pt]
24 & 0.03 & $-$0.52 & 0.65 & $-$0.51 & $-$0.01 \\
\footnotesize & [$-$0.16, 0.17] & [$-$0.75, $-$0.25] & & [$-$0.69, $-$0.24] & [$-$0.03, 0.00] \\[2pt]
36 & $-$0.02 & $-$0.68 & 0.70 & $-$0.61 & $-$0.01 \\
\footnotesize & [$-$0.24, 0.13] & [$-$0.93, $-$0.40] & & [$-$0.79, $-$0.33] & [$-$0.04, $-$0.00] \\[2pt]
\bottomrule
\end{tabular}
\par\smallskip\parbox{0.95\textwidth}{\footnotesize Average across the 37 states with at least twelve months of EB, October 2002 to December 2019. Cumulated response in percentage points to an EB innovation of ten weeks, with EUC ordered first. CVAR: VAR in the weeks of EUC and EB and the change in the cycle, equal weights on the controls. VAR without controls: the same with the change in the unemployment rate of the treated state. Weighted controls: response in the VAR with both the treated state and the weighted controls (Proposition \ref{prop:placebo}). Impulse causal effect of one week of EB from Theorem \ref{thm:direct}. 6 lags in every state; 90 percent bands from 999 draws of a residual bootstrap that draws the same months for every state.}
\end{table}


==> exhibits/tab_eb_bounds.tex <==
\begin{table}[htbp]
\centering
\caption{Sensitivity to the exogeneity assumption, average across states\label{tab:eb-bounds}}
\small
\begin{tabular}{cccccc}
\toprule
Months & VAR with controls added & $\lambda=0$ & $\lambda=0.25$ & $\lambda=0.5$ & $\lambda$ reaching the VAR \\
\midrule
6 & $-$0.22 & [$-$0.03, 0.09] & [$-$0.09, 0.16] & [$-$0.16, 0.23] & 0.70 \\
12 & $-$0.34 & [$-$0.06, 0.14] & [$-$0.15, 0.22] & [$-$0.26, 0.33] & 0.66 \\
\bottomrule
\end{tabular}
\par\smallskip\parbox{0.95\textwidth}{\footnotesize Response of the treated state in the VAR with the weighted controls added, and 90 percent bands for the bounds of Proposition \ref{prop:bounds}, with the bias specific to the treated state at most $\lambda$ times the bias from the common trends. Last column: smallest $\lambda$ at which the band contains the response of the treated state.}
\end{table}


==> exhibits/tab_eb_lpdid.tex <==
\begin{table}[htbp]
\centering
\caption{Extended benefits: local-projection difference-in-differences and the CVAR\label{tab:eb-lpdid}}
\small
\begin{tabular}{ccccc}
\toprule
 & \multicolumn{2}{c}{LP difference-in-differences} & \multicolumn{2}{c}{VAR responses} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
Months & Never-triggered controls & Clean controls & CVAR & VAR without controls \\
\midrule
0 & 0.07 [0.02, 0.12] & $-$0.01 [$-$0.05, 0.03] & $-$0.00 [$-$0.02, 0.01] & $-$0.03 [$-$0.05, $-$0.01] \\
6 & 0.46 [0.10, 0.82] & 0.22 [$-$0.14, 0.58] & 0.03 [$-$0.03, 0.11] & $-$0.23 [$-$0.32, $-$0.11] \\
12 & 0.37 [$-$0.08, 0.81] & 0.10 [$-$0.33, 0.53] & 0.05 [$-$0.06, 0.17] & $-$0.33 [$-$0.47, $-$0.13] \\
24 & 0.31 [$-$0.17, 0.79] & $-$0.07 [$-$0.58, 0.44] & 0.03 [$-$0.16, 0.17] & $-$0.52 [$-$0.75, $-$0.25] \\
36 & 0.62 [0.08, 1.16] & $-$0.07 [$-$0.77, 0.63] & $-$0.02 [$-$0.24, 0.13] & $-$0.68 [$-$0.93, $-$0.40] \\
\bottomrule
\end{tabular}
\par\smallskip\parbox{0.95\textwidth}{\footnotesize Change in the unemployment rate in percentage points. LP difference-in-differences \citep{dube2023local}: response to EB switching on in a state (38 events with no EB in the previous twelve months), with month fixed effects, four lags of the change in the unemployment rate and the current value and four lags of the change in the weeks of EUC; controls are the never-triggered states, or every state-month without EB in the twelve months before the event and up to the horizon. The coefficients are divided by the average size of a switch-on, 0.90 tens of weeks, to express them per ten weeks; 90 percent bands from standard errors clustered by state. CVAR and VAR without controls: average response to an EB innovation of ten weeks, from Table \ref{tab:eb-avg}.}
\end{table}


==> exhibits/tab_eb_states.tex <==
\begin{table}[htbp]
\centering
\caption{Response of the unemployment rate to ten additional weeks of EB after twelve months, by state\label{tab:eb-states}}
\small
\begin{tabular}{lcccc}
\toprule
State & Lags & CVAR & VAR without controls & Width ratio \\
\midrule
AK & 7/9 & $-$0.05 [$-$0.19, 0.14] & $-$0.12 [$-$0.31, 0.07] & 0.86 \\
AL & 8/8 & $-$0.64 [$-$1.20, 0.00] & $-$1.06 [$-$1.75, $-$0.23] & 0.79 \\
AZ & 11/11 & 0.04 [$-$0.47, 0.55] & $-$0.39 [$-$1.01, 0.34] & 0.76 \\
CA & 4/6 & 0.12 [$-$0.21, 0.53] & $-$0.55 [$-$1.00, 0.17] & 0.63 \\
CO & 7/8 & 0.07 [$-$0.53, 0.70] & $-$0.32 [$-$1.02, 0.46] & 0.83 \\
CT & 3/3 & 0.56 [0.09, 0.93] & 0.11 [$-$0.92, 0.57] & 0.56 \\
DE & 8/12 & 0.15 [$-$0.21, 0.57] & $-$0.07 [$-$0.74, 0.66] & 0.56 \\
FL & 8/8 & $-$0.13 [$-$0.46, 0.24] & $-$0.46 [$-$0.91, 0.11] & 0.68 \\
GA & 3/3 & 0.30 [$-$0.20, 0.69] & $-$0.30 [$-$0.89, 0.35] & 0.73 \\
ID & 7/5 & 0.37 [$-$0.32, 1.10] & 0.03 [$-$0.95, 1.05] & 0.71 \\
IL & 3/7 & 0.02 [$-$0.45, 0.43] & $-$0.41 [$-$1.03, 0.31] & 0.66 \\
IN & 8/8 & $-$0.14 [$-$0.71, 0.44] & $-$1.01 [$-$1.91, $-$0.04] & 0.61 \\
KS & 2/7 & $-$0.06 [$-$0.43, 0.33] & $-$0.50 [$-$1.27, 0.25] & 0.50 \\
KY & 3/6 & $-$0.46 [$-$0.83, 0.02] & $-$0.86 [$-$1.45, $-$0.11] & 0.64 \\
MA & 7/7 & 0.17 [$-$0.28, 0.61] & $-$0.52 [$-$1.14, 0.17] & 0.67 \\
ME & 8/8 & 0.02 [$-$0.42, 0.49] & $-$0.91 [$-$1.57, $-$0.06] & 0.60 \\
MI & 2/7 & $-$0.84 [$-$1.38, $-$0.16] & $-$1.63 [$-$2.42, $-$0.55] & 0.65 \\
MN & 2/2 & $-$0.36 [$-$0.80, 0.20] & $-$1.10 [$-$1.93, $-$0.45] & 0.67 \\
MO & 7/6 & $-$0.10 [$-$0.31, 0.12] & $-$0.23 [$-$0.62, 0.18] & 0.53 \\
NC & 1/1 & 0.41 [$-$0.02, 0.71] & 0.53 [$-$0.20, 0.99] & 0.61 \\
NH & 1/2 & $-$0.27 [$-$0.81, 0.13] & $-$0.49 [$-$1.37, 0.08] & 0.65 \\
NJ & 2/2 & 0.92 [0.09, 1.71] & 0.37 [$-$1.03, 0.94] & 0.82 \\
NM & 3/2 & $-$0.14 [$-$0.67, 0.35] & $-$0.51 [$-$1.36, 0.17] & 0.66 \\
NV & 2/2 & 0.42 [$-$0.23, 1.02] & $-$0.28 [$-$1.05, 0.40] & 0.87 \\
NY & 4/4 & 0.19 [$-$0.15, 0.50] & 0.13 [$-$0.42, 0.52] & 0.70 \\
OH & 8/8 & $-$0.40 [$-$0.77, 0.04] & $-$1.09 [$-$1.72, $-$0.24] & 0.55 \\
OR & 5/5 & 0.06 [$-$0.49, 0.47] & 0.10 [$-$0.69, 0.91] & 0.60 \\
PA & 7/8 & 0.11 [$-$0.07, 0.31] & $-$0.28 [$-$0.78, 0.22] & 0.39 \\
RI & 2/2 & $-$0.09 [$-$0.78, 1.10] & 0.49 [$-$0.36, 1.88] & 0.84 \\
SC & 9/8 & 0.38 [$-$0.15, 0.93] & $-$0.08 [$-$0.74, 0.82] & 0.69 \\
TN & 5/4 & $-$0.23 [$-$0.57, 0.16] & $-$0.37 [$-$0.86, 0.18] & 0.70 \\
TX & 7/11 & $-$0.24 [$-$0.60, 0.13] & $-$1.57 [$-$2.27, $-$0.70] & 0.46 \\
VA & 5/5 & $-$0.15 [$-$0.57, 0.33] & $-$0.31 [$-$1.11, 0.51] & 0.56 \\
VT & 2/2 & $-$0.34 [$-$0.78, 0.19] & $-$0.90 [$-$1.66, 0.01] & 0.58 \\
WA & 1/2 & 0.48 [0.05, 0.81] & $-$0.01 [$-$0.77, 0.61] & 0.56 \\
WI & 9/9 & $-$0.47 [$-$0.86, 0.05] & $-$0.63 [$-$1.41, 0.16] & 0.58 \\
WV & 11/11 & $-$0.18 [$-$0.61, 0.22] & $-$0.74 [$-$1.53, 0.14] & 0.50 \\
\bottomrule
\end{tabular}
\par\smallskip\parbox{0.95\textwidth}{\footnotesize Cumulated response in percentage points, with 90 percent bands from 999 residual bootstrap draws. Lags: CVAR / VAR without controls, chosen by the rule of Section \ref{sec:eb}. Width ratio: width of the CVAR band over that of the VAR without controls.}
\end{table}


==> exhibits/tab_eb_tests.tex <==
\begin{table}[htbp]
\centering
\caption{Unit roots and the test of the design\label{tab:eb-tests}}
\small
\begin{tabular}{llcc}
\toprule
Series & Specification & Rejections at 5 percent & Median p-value \\
\midrule
Unemployment rate, treated states & ERS & 4 of 37 & 0.09 \\
Unemployment rate, controls & ERS & 2 of 7 & 0.08 \\
\midrule
Cycle, estimated weights, no level shifts & $q=12$ & 0 of 37 & 0.20 \\
Cycle, estimated weights, no level shifts & $q=6$ & 0 of 37 & 0.23 \\
Cycle, estimated weights, no level shifts & $q=3$ & 1 of 37 & 0.22 \\
Cycle, estimated weights, no level shifts & $q=0$ & 0 of 37 & 0.21 \\
Cycle, estimated weights, level shifts & $q=12$ & 0 of 37 & 0.21 \\
Cycle, estimated weights, level shifts & $q=6$ & 0 of 37 & 0.24 \\
Cycle, estimated weights, level shifts & $q=3$ & 1 of 37 & 0.22 \\
Cycle, estimated weights, level shifts & $q=0$ & 0 of 37 & 0.21 \\
\midrule
Cycle, equal weights & $q=12$ & 0 of 37 & 0.20 \\
Cycle, equal weights, no policy terms & & 1 of 37 & 0.19 \\
\bottomrule
\end{tabular}
\par\smallskip\parbox{0.95\textwidth}{\footnotesize ERS: point-optimal test of \citet{ERS1996} with a constant, on the unemployment rate. Cycle: test of Section \ref{sec:test} of the null that the treated state has a stochastic trend of its own, with the current value and $q$ lags of the weeks of EUC and EB, controls the never-triggered states that do not border the treated state, weights estimated by \eqref{eq:dols} or set equal. Level shifts: sequential sup-Wald tests on the cycle net of the policy terms. Sieve-bootstrap p-values.}
\end{table}


==> exhibits/tab_mc_boot.tex <==
\begin{table}[H]
\centering
\caption{Average coverage of the 90 percent bands for $\gamma_h$ across the designs of the grid, with 12 lags, 500 replications per design and 499 bootstrap draws. 8 designs without feedback ($\phi=0$) and 9 with feedback ($\phi=0.3$).\label{tab:mc-boot}}
\begin{tabular}{r ccc c ccc}
\toprule
 & \multicolumn{3}{c}{$\phi=0$} & & \multicolumn{3}{c}{$\phi=0.3$}\\
\cmidrule{2-4}\cmidrule{6-8}
$h$ & Known & Fixed & Re-estimated & & Known & Fixed & Re-estimated\\
\midrule
0 & 0.89 & 0.88 & 0.89 &  & 0.89 & 0.88 & 0.89\\
1 & 0.89 & 0.88 & 0.89 &  & 0.90 & 0.88 & 0.90\\
3 & 0.89 & 0.87 & 0.88 &  & 0.89 & 0.87 & 0.88\\
6 & 0.88 & 0.87 & 0.88 &  & 0.87 & 0.88 & 0.88\\
12 & 0.89 & 0.88 & 0.89 &  & 0.89 & 0.88 & 0.90\\
24 & 0.99 & 0.99 & 0.99 &  & 0.82 & 0.80 & 0.80\\
\bottomrule
\end{tabular}
\end{table}


==> exhibits/tab_mc_diff.tex <==
\begin{table}[htbp]
\centering
\caption{The CVAR in changes with imposed weights\label{tab:mc-diff}}
\small
\begin{tabular}{lccccccc}
\toprule
 & \multicolumn{3}{c}{Bias} & \multicolumn{3}{c}{Coverage} & Width \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-8}
Horizon & 0 & 6 & 12 & 0 & 6 & 12 & 6 \\
\midrule
\multicolumn{8}{l}{Trend of the treated unit} \\
CVAR in changes & $-$0.00 & $-$0.02 & 0.00 & 0.91 & 0.85 & 0.92 & 0.28 \\
VAR without controls & 0.50 & 0.46 & 0.48 & 0.00 & 0.20 & 0.06 & 0.59 \\
CVAR in levels & $-$0.00 & $-$0.03 & 0.00 & 0.69 & 0.79 & 0.89 & 0.29 \\
\midrule
\multicolumn{8}{l}{Stationary cycle} \\
CVAR in changes & 0.00 & $-$0.00 & 0.02 & 0.87 & 0.91 & 0.95 & 0.31 \\
VAR without controls & 0.50 & 0.48 & 0.50 & 0.00 & 0.21 & 0.08 & 0.61 \\
CVAR in levels & 0.00 & $-$0.02 & $-$0.00 & 0.89 & 0.84 & 0.94 & 0.26 \\
\midrule
\multicolumn{8}{l}{One noisy control} \\
CVAR in changes & 0.00 & 0.01 & 0.08 & 0.90 & 0.96 & 0.94 & 0.59 \\
VAR without controls & 0.50 & 0.46 & 0.48 & 0.00 & 0.24 & 0.08 & 0.59 \\
CVAR in levels & 0.06 & 0.02 & 0.02 & 0.66 & 0.90 & 0.95 & 0.40 \\
\midrule
\multicolumn{8}{l}{No reaction to the common shock} \\
CVAR in changes & $-$0.00 & $-$0.01 & 0.01 & 0.89 & 0.90 & 0.93 & 0.32 \\
VAR without controls & 0.00 & $-$0.02 & 0.00 & 0.89 & 0.89 & 0.89 & 0.65 \\
CVAR in levels & $-$0.00 & $-$0.03 & 0.00 & 0.92 & 0.85 & 0.94 & 0.31 \\
\bottomrule
\end{tabular}
\par\smallskip\parbox{0.95\textwidth}{\footnotesize 500 replications, $T=200$, 4 lags, 199 bootstrap draws in each replication. Cumulated response to a unit innovation in the policy; bias relative to the true response, coverage of 90 percent percentile bands, and mean width of the band. Data generating process and designs in the text.}
\end{table}


==> exhibits/tab_mc_grid.tex <==
\begin{table}[H]
\centering\small
\caption{Coverage of the 90 percent bands for $\gamma_h$ in every design of the grid of Appendix \ref{sec:montecarlo}, on impact and after twelve months. Known: weights known. Fixed: estimated weights held fixed. Re-est.: weights re-estimated in every draw. Boundary: one true weight equal to zero.\label{tab:mc-grid}}
\begin{tabular}{ccccc ccc ccc}
\toprule
 & & & & & \multicolumn{3}{c}{$h=0$} & \multicolumn{3}{c}{$h=12$}\\
\cmidrule{6-8}\cmidrule{9-11}
$T$ & $K$ & $r$ & $\phi$ & Boundary & Known & Fixed & Re-est. & Known & Fixed & Re-est.\\
\midrule
200 & 3 & 2 & 0.0 & no & 0.90 & 0.88 & 0.89 & 0.89 & 0.88 & 0.88\\
200 & 3 & 2 & 0.3 & no & 0.90 & 0.89 & 0.89 & 0.88 & 0.87 & 0.90\\
200 & 3 & 3 & 0.0 & no & 0.90 & 0.87 & 0.89 & 0.91 & 0.89 & 0.90\\
200 & 3 & 3 & 0.3 & yes & 0.87 & 0.89 & 0.89 & 0.90 & 0.89 & 0.91\\
200 & 3 & 3 & 0.3 & no & 0.90 & 0.88 & 0.89 & 0.89 & 0.88 & 0.90\\
200 & 6 & 5 & 0.0 & no & 0.87 & 0.85 & 0.87 & 0.90 & 0.89 & 0.90\\
200 & 6 & 5 & 0.3 & no & 0.91 & 0.86 & 0.87 & 0.88 & 0.89 & 0.91\\
200 & 6 & 6 & 0.0 & no & 0.91 & 0.88 & 0.90 & 0.90 & 0.87 & 0.89\\
200 & 6 & 6 & 0.3 & no & 0.88 & 0.86 & 0.88 & 0.87 & 0.85 & 0.87\\
400 & 3 & 2 & 0.0 & no & 0.89 & 0.88 & 0.89 & 0.89 & 0.90 & 0.91\\
400 & 3 & 2 & 0.3 & no & 0.90 & 0.89 & 0.90 & 0.91 & 0.91 & 0.92\\
400 & 3 & 3 & 0.0 & no & 0.90 & 0.90 & 0.90 & 0.86 & 0.88 & 0.88\\
400 & 3 & 3 & 0.3 & no & 0.90 & 0.89 & 0.89 & 0.91 & 0.91 & 0.92\\
400 & 6 & 5 & 0.0 & no & 0.90 & 0.89 & 0.89 & 0.90 & 0.89 & 0.89\\
400 & 6 & 5 & 0.3 & no & 0.91 & 0.87 & 0.89 & 0.87 & 0.86 & 0.88\\
400 & 6 & 6 & 0.0 & no & 0.88 & 0.86 & 0.89 & 0.88 & 0.87 & 0.88\\
400 & 6 & 6 & 0.3 & no & 0.88 & 0.88 & 0.88 & 0.88 & 0.89 & 0.90\\
\bottomrule
\end{tabular}
\end{table}


==> exhibits/tab_mc_joint.tex <==
\begin{table}[htbp]
\centering
\caption{Coverage of the 90 percent bands for $\gamma_h$ with estimated weights: bootstrap schemes\label{tab:mc-joint}}
\small
\begin{tabular}{lccccccc}
\toprule
 & \multicolumn{6}{c}{Coverage, months after the surprise} & Width \\
\cmidrule(lr){2-7}\cmidrule(lr){8-8}
 & 0 & 1 & 3 & 6 & 12 & 24 & 12 \\
\midrule
\multicolumn{8}{l}{$T=200$, $\phi=0.3$} \\
Known weights & 0.89 & 0.89 & 0.90 & 0.85 & 0.89 & 0.85 & 0.41 \\
Fixed weights & 0.87 & 0.88 & 0.88 & 0.84 & 0.87 & 0.81 & 0.38 \\
Re-estimated, controls fixed & 0.90 & 0.89 & 0.89 & 0.86 & 0.91 & 0.83 & 0.40 \\
Joint, not recentred & 0.90 & 0.89 & 0.89 & 0.85 & 0.89 & 0.81 & 0.40 \\
Joint, recentred (Theorem \ref{thm:joint}) & 0.89 & 0.88 & 0.88 & 0.85 & 0.88 & 0.82 & 0.40 \\
\midrule
\multicolumn{8}{l}{$T=200$, $\phi=0.45$} \\
Known weights & 0.90 & 0.89 & 0.90 & 0.84 & 0.86 & 0.61 & 0.47 \\
Fixed weights & 0.88 & 0.87 & 0.88 & 0.86 & 0.87 & 0.61 & 0.44 \\
Re-estimated, controls fixed & 0.90 & 0.89 & 0.89 & 0.87 & 0.91 & 0.64 & 0.44 \\
Joint, not recentred & 0.90 & 0.89 & 0.90 & 0.85 & 0.90 & 0.64 & 0.45 \\
Joint, recentred (Theorem \ref{thm:joint}) & 0.88 & 0.87 & 0.89 & 0.83 & 0.88 & 0.63 & 0.45 \\
\midrule
\multicolumn{8}{l}{$T=400$, $\phi=0.3$} \\
Known weights & 0.88 & 0.89 & 0.90 & 0.87 & 0.90 & 0.77 & 0.28 \\
Fixed weights & 0.88 & 0.89 & 0.89 & 0.86 & 0.89 & 0.75 & 0.27 \\
Re-estimated, controls fixed & 0.88 & 0.90 & 0.89 & 0.87 & 0.90 & 0.75 & 0.27 \\
Joint, not recentred & 0.89 & 0.90 & 0.90 & 0.88 & 0.90 & 0.76 & 0.28 \\
Joint, recentred (Theorem \ref{thm:joint}) & 0.88 & 0.90 & 0.90 & 0.89 & 0.88 & 0.76 & 0.28 \\
\bottomrule
\end{tabular}
\par\smallskip\parbox{0.95\textwidth}{\footnotesize Six controls with one cointegrating relation among them, feedback $\phi$ from the lagged cycle to the policy, 12 lags in the VAR of the CVAR and in the joint VAR, 500 replications and 499 bootstrap draws. Known weights: pseudo-true weights. Fixed weights: estimated weights held fixed. Re-estimated, controls fixed: weights re-estimated in every draw with the controls at their observed values. Joint: the controls are regenerated with the policies and the cycle and the weights re-estimated, without recentring, or with the draws recentred at the response of the bootstrap world as in Theorem \ref{thm:joint}.}
\end{table}


==> exhibits/tab_mc_lags.tex <==
\begin{table}[H]
\centering
\caption{CVAR with different lag lengths. Bias of the response and coverage of the 90 percent bands for $\gamma_h$, bootstrap with re-estimated weights. $T=200$, $K=6$, $r=5$, $\phi=0.3$, 500 replications.\label{tab:mc-lags}}
\begin{tabular}{rr cc cc cc}
\toprule
 & & \multicolumn{2}{c}{Akaike (mean 1.3)} & \multicolumn{2}{c}{8 lags} & \multicolumn{2}{c}{12 lags}\\
$h$ & $\gamma_h$ & Bias & Coverage & Bias & Coverage & Bias & Coverage\\
\midrule
0 & 0.198 & $-$0.002 & 0.91 & 0.001 & 0.90 & 0.003 & 0.90\\
1 & 0.267 & 0.046 & 0.79 & $-$0.002 & 0.89 & 0.001 & 0.89\\
3 & 0.282 & 0.006 & 0.83 & $-$0.004 & 0.90 & 0.001 & 0.89\\
6 & 0.231 & $-$0.061 & 0.57 & $-$0.010 & 0.88 & $-$0.006 & 0.86\\
12 & 0.154 & $-$0.093 & 0.24 & $-$0.046 & 0.75 & $-$0.004 & 0.91\\
24 & 0.067 & $-$0.056 & 0.13 & $-$0.041 & 0.60 & $-$0.040 & 0.83\\
\bottomrule
\end{tabular}
\end{table}


==> exhibits/tab_mc_nonlin.tex <==
\begin{table}[H]
\centering\small
\caption{Non-linear effects. Bias at impact and after three months, and root mean squared error averaged over horizons 0 to 12, for the response to a policy innovation of size $\delta$, with the effect $u+\kappa u^2$. $\delta$ equal to minus one, one and two standard deviations of the innovation, $T=200$, 1000 replications, 12 lags.\label{tab:mc-nonlin}}
\begin{tabular}{cc ccc ccc}
\toprule
 & & \multicolumn{3}{c}{Linear CVAR} & \multicolumn{3}{c}{Dictionary, Theorem \ref{thm:nonlin}}\\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}
$\kappa$ & $\delta$ & Bias $h=0$ & Bias $h=3$ & RMSE & Bias $h=0$ & Bias $h=3$ & RMSE\\
\midrule
0.0 & -1.12 & $-$0.005 & 0.002 & 0.104 & $-$0.012 & 0.003 & 0.140\\
0.0 & 1.12 & 0.005 & $-$0.002 & 0.104 & $-$0.002 & $-$0.000 & 0.140\\
0.0 & 2.24 & 0.009 & $-$0.003 & 0.209 & $-$0.018 & 0.002 & 0.411\\
0.5 & -1.12 & $-$0.130 & $-$0.062 & 0.132 & $-$0.019 & $-$0.012 & 0.145\\
0.5 & 1.12 & $-$0.120 & $-$0.066 & 0.132 & $-$0.010 & $-$0.017 & 0.143\\
0.5 & 2.24 & $-$0.491 & $-$0.260 & 0.361 & $-$0.049 & $-$0.064 & 0.424\\
\bottomrule
\end{tabular}
\end{table}


==> exhibits/tab_mc_spill.tex <==
\begin{table}[H]
\centering\small
\caption{Spillovers. Bias at impact ($h=0$) and after three months ($h=3$), and root mean squared error averaged over horizons 0 to 12, for the effect of a policy surprise. Five controls at increasing distance, exposure $x_k=(d_1/d_k)^2$, $T=200$, 1000 replications, 12 lags.\label{tab:mc-spill}}
\begin{tabular}{l ccc ccc}
\toprule
 & \multicolumn{3}{c}{No spillover, $\pi=0$} & \multicolumn{3}{c}{Spillover, $\pi=0.5$}\\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Estimator & $h=0$ & $h=3$ & RMSE & $h=0$ & $h=3$ & RMSE\\
\midrule
CVAR, all controls & 0.002 & $-$0.006 & 0.091 & $-$0.026 & $-$0.037 & 0.094\\
CVAR, nearest control & 0.013 & $-$0.002 & 0.142 & $-$0.109 & $-$0.134 & 0.173\\
CVAR, most distant control & 0.004 & $-$0.009 & 0.120 & $-$0.002 & $-$0.014 & 0.119\\
Exposure estimator & 0.004 & $-$0.008 & 0.106 & 0.004 & $-$0.008 & 0.106\\
\bottomrule
\end{tabular}
\end{table}


==> exhibits/tab_mc_stat.tex <==
\begin{table}[H]
\centering\small
\caption{Stationarity diagnostics for the estimated cycle. Rejection frequencies at 5 percent with the standard critical values (Engle-Granger for ADF, 0.463 for KPSS) and with simulated critical values (from the unit-root design for ADF and from the design with $\rho=0.9$ for KPSS). $\rho=1$: the counterfactual cycle has a unit root. $\rho=0.9$: it is a stationary AR(1). The ADF test takes a unit root as the null hypothesis, the KPSS test stationarity. Six controls, weights estimated by constrained dynamic least squares with policy terms, 1000 replications.\label{tab:mc-stat}}
\begin{tabular}{ll cc cc}
\toprule
 & & \multicolumn{2}{c}{Standard critical values} & \multicolumn{2}{c}{Simulated critical values}\\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
$T$ & Statistic & $\rho=1$ & $\rho=0.9$ & $\rho=1$ & $\rho=0.9$\\
\midrule
200 & ADF, cycle & 0.22 & 0.77 & 0.05 & 0.33\\
200 & ADF, cycle net of policy & 0.47 & 0.94 & 0.05 & 0.33\\
200 & KPSS, cycle & 0.18 & 0.06 & 0.17 & 0.05\\
200 & KPSS, cycle net of policy & 0.09 & 0.00 & 0.37 & 0.05\\
400 & ADF, cycle & 0.36 & 0.99 & 0.05 & 0.86\\
400 & ADF, cycle net of policy & 0.45 & 1.00 & 0.05 & 0.89\\
400 & KPSS, cycle & 0.25 & 0.02 & 0.37 & 0.05\\
400 & KPSS, cycle net of policy & 0.19 & 0.00 & 0.64 & 0.05\\
\bottomrule
\end{tabular}
\end{table}


==> exhibits/tab_mc_var.tex <==
\begin{table}[H]
\centering
\caption{VAR without controls and CVAR, both with 12 lags. Bias, root mean squared error and coverage of the 90 percent bands for the effect of a policy surprise $\theta_h$. $T=200$, $K=6$, $r=5$, $\phi=0.3$, 500 replications, 499 bootstrap draws.\label{tab:mc-var}}
\begin{tabular}{rr ccc c ccc}
\toprule
 & & \multicolumn{3}{c}{VAR without controls} & & \multicolumn{3}{c}{CVAR}\\
\cmidrule{3-5}\cmidrule{7-9}
$h$ & $\theta_h$ & Bias & RMSE & Coverage & & Bias & RMSE & Coverage\\
\midrule
0 & 0.200 & 0.185 & 0.213 & 0.49 & & 0.001 & 0.082 & 0.90\\
1 & 0.272 & 0.215 & 0.267 & 0.62 & & $-$0.005 & 0.097 & 0.90\\
3 & 0.285 & 0.203 & 0.312 & 0.81 & & $-$0.002 & 0.109 & 0.89\\
6 & 0.236 & 0.160 & 0.351 & 0.88 & & $-$0.010 & 0.128 & 0.86\\
12 & 0.152 & 0.125 & 0.413 & 0.87 & & $-$0.002 & 0.129 & 0.91\\
24 & 0.068 & 0.085 & 0.417 & 0.91 & & $-$0.041 & 0.084 & 0.82\\
\bottomrule
\end{tabular}
\end{table}


==> exhibits/tab_screen.tex <==
\begin{table}[htbp]
\centering
\caption{The test of the design on US states, regions and metropolitan areas\label{tab:screen}}
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{>{\raggedright\arraybackslash}p{4.2cm}cccccc}
\toprule
 & Units & Observations & \multicolumn{3}{c}{Share rejecting at 5 percent} & Gap stationary, \\
\cmidrule(lr){4-6}
 & & & Alone & Equal & Estimated & series I(1) \\
\midrule
Employment-population ratio & 49 & 528 months & 0.00 & 0.08 & 0.10 & 7 \\
Participation rate & 49 & 528 months & 0.00 & 0.14 & 0.04 & 8 \\
Payroll employment & 49 & 360 months & 0.00 & 0.02 & 0.00 & 1 \\
Coincident index & 48 & 492 months & 0.00 & 0.00 & 0.02 & 1 \\
Personal income & 49 & 288 quarters & 0.02 & 0.02 & 0.00 & 1 \\
House prices & 49 & 180 quarters & 0.00 & 0.04 & 0.02 & 3 \\
Consumer prices, Census regions & 4 & 495 months & 0.00 & 0.00 & 0.00 & 0 \\
Consumer prices, three metropolitan areas & 3 & 993 months & 0.00 & 0.00 & 0.00 & 0 \\
\bottomrule
\end{tabular}
\par\smallskip\parbox{0.95\textwidth}{\footnotesize Test of Section \ref{sec:test} with a constant and no policy terms, sieve-bootstrap p-values with 499 draws. The 48 contiguous states and the District of Columbia, each against the states it borders; consumer prices for each Census region against the other three, and for New York, Chicago and Los Angeles against the other two. Observations: median sample length, from the start of each series (1976 for the employment-population ratio and the participation rate, 1990 for payroll employment, 1979 for the coincident index, 1948 for personal income, 1975 for house prices, 1966 for the regions and 1914 for the metropolitan areas) to the end of 2019. Alone: the unit without controls. Equal: the unit minus the average of its neighbours. Estimated: weights on the neighbours estimated inside the test. Last column: number of units for which the unit alone does not reject at 10 percent and the gap with the neighbours rejects at 5 percent with equal or estimated weights.}
\end{table}


==> exhibits/tab_screen_power.tex <==
\begin{table}[htbp]
\centering
\caption{Size and power of the test of the design in panels built like the state data\label{tab:screen-power}}
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcccccccc}
\toprule
Sample & Half-life & $c$ & \multicolumn{3}{c}{Equal weights} & \multicolumn{2}{c}{Estimated weights} \\
\cmidrule(lr){4-6}\cmidrule(lr){7-8}
 & (years) & & Bootstrap & Residual & ERS & Bootstrap & Residual \\
\midrule
15 years & trend of its own & -- & 0.05 & 0.12 & 0.08 & 0.05 & 0.13 \\
 & 1.1 & $-$9.0 & 0.20 & 0.37 & 0.38 & 0.16 & 0.35 \\
 & 2.9 & $-$3.6 & 0.09 & 0.19 & 0.14 & 0.07 & 0.19 \\
 & 5.7 & $-$1.8 & 0.07 & 0.16 & 0.10 & 0.04 & 0.19 \\
 & 11.5 & $-$0.9 & 0.04 & 0.11 & 0.06 & 0.03 & 0.12 \\
\addlinespace
25 years & trend of its own & -- & 0.06 & 0.12 & 0.09 & 0.04 & 0.11 \\
 & 1.1 & $-$15.0 & 0.40 & 0.59 & 0.56 & 0.26 & 0.56 \\
 & 2.9 & $-$6.0 & 0.15 & 0.30 & 0.24 & 0.13 & 0.30 \\
 & 5.7 & $-$3.0 & 0.08 & 0.18 & 0.13 & 0.09 & 0.17 \\
 & 11.5 & $-$1.5 & 0.05 & 0.13 & 0.09 & 0.04 & 0.13 \\
\addlinespace
44 years & trend of its own & -- & 0.08 & 0.12 & 0.09 & 0.03 & 0.08 \\
 & 1.1 & $-$26.4 & 0.63 & 0.82 & 0.82 & 0.46 & 0.69 \\
 & 2.9 & $-$10.6 & 0.37 & 0.54 & 0.50 & 0.29 & 0.48 \\
 & 5.7 & $-$5.3 & 0.16 & 0.28 & 0.25 & 0.13 & 0.27 \\
 & 11.5 & $-$2.6 & 0.07 & 0.14 & 0.10 & 0.08 & 0.17 \\
\bottomrule
\end{tabular}
\par\smallskip\parbox{0.95\textwidth}{\footnotesize Rejection rates at 5 percent in 300 replications of monthly panels with one common stochastic trend, four controls that load on it with stationary noise, and a treated unit that follows the common trend plus a gap: a random walk (trend of its own: the rows give the size) or a stationary autoregression with the half-life shown, $c=T(\rho-1)$. Bootstrap: the sieve bootstrap of Proposition \ref{prop:sieve}, 199 draws. Residual: a sieve bootstrap that takes the innovations from the unrestricted autoregression in levels and imposes the unit root when rebuilding the series \citep{PaparoditisPolitis2003,PalmSmeekesUrbain2008}. ERS: the asymptotic critical value of \citet{ERS1996}, valid only without estimated weights.}
\end{table}


==> exhibits/table11.tex <==
\begin{table}[H]
\centering\small
\caption{Test of the design: rejection rates under the null ($g=0$) at the 5 percent level. CVAR test: statistic \eqref{eq:PT} with $\bar c=-7$ and the critical value of \citet{ERS1996}; bootstrap: sieve bootstrap p-value with an autoregression of order $p_T=\lceil16(T/200)^{1/3}\rceil$; robust: adaptive test of Appendix \ref{sec:supp-test}, with the critical value from the null with uncorrelated innovations of the same design, so that its size is nominal by construction when $\delta=0$; PR: ADF-GLS of \citet{PerronRodriguez2016} with their critical values (not tabulated for six regressors); EG: Engle-Granger with the critical values of \citet{MacKinnon2010}; Johansen: maximum eigenvalue test. $\delta$: correlation between the innovations of the cycle and those of the controls. 1000 replications, 199 bootstrap draws.\label{tab:mc-test-size}}
\begin{tabular}{rlc cccccc}
\toprule
$T$ & Design & $\delta$ & CVAR test & Bootstrap & Robust & PR & EG & Johansen\\
\midrule
200 & Triangular, $k=1$ & 0.0 & 0.046 & 0.027 & 0.050 & 0.039 & 0.036 & 0.054\\
200 & Triangular, $k=1$ & 0.6 & 0.058 & 0.031 & 0.063 & 0.044 & 0.042 & 0.087\\
200 & Triangular, $k=3$ & 0.0 & 0.050 & 0.028 & 0.050 & 0.040 & 0.050 & 0.071\\
200 & Triangular, $k=3$ & 0.6 & 0.032 & 0.018 & 0.036 & 0.029 & 0.030 & 0.062\\
200 & CVAR, $K=3$ & 0.0 & 0.089 & 0.061 & 0.050 & 0.078 & 0.256 & 0.108\\
200 & CVAR, $K=3$ & 0.6 & 0.093 & 0.055 & 0.045 & 0.077 & 0.290 & 0.112\\
200 & CVAR, $K=6$ & 0.0 & 0.071 & 0.040 & 0.050 &  & 0.262 & 0.822\\
200 & CVAR, $K=6$ & 0.6 & 0.091 & 0.045 & 0.058 &  & 0.311 & 0.815\\
400 & Triangular, $k=1$ & 0.0 & 0.053 & 0.033 & 0.050 & 0.046 & 0.061 & 0.072\\
400 & Triangular, $k=1$ & 0.6 & 0.035 & 0.030 & 0.031 & 0.042 & 0.037 & 0.056\\
400 & Triangular, $k=3$ & 0.0 & 0.043 & 0.029 & 0.050 & 0.045 & 0.043 & 0.056\\
400 & Triangular, $k=3$ & 0.6 & 0.055 & 0.032 & 0.055 & 0.045 & 0.049 & 0.061\\
400 & CVAR, $K=3$ & 0.0 & 0.066 & 0.047 & 0.050 & 0.068 & 0.288 & 0.086\\
400 & CVAR, $K=3$ & 0.6 & 0.090 & 0.054 & 0.052 & 0.090 & 0.341 & 0.097\\
400 & CVAR, $K=6$ & 0.0 & 0.093 & 0.055 & 0.050 &  & 0.317 & 1.000\\
400 & CVAR, $K=6$ & 0.6 & 0.083 & 0.059 & 0.041 &  & 0.392 & 1.000\\
\bottomrule
\end{tabular}
\end{table}


==> exhibits/table12.tex <==
\begin{table}[H]
\centering\small
\caption{Test of the design: size-adjusted power at the local alternative $\rho=1-10/T$. Bound: power of the Neyman-Pearson test that knows the weights and the covariance \citep{ElliottJanssonPesavento2005}, computed in the triangular designs. ECR: error-correction $t$-test; Wald: \citet{Boswijk1994}. Other columns as in Table \ref{tab:mc-test-size}.\label{tab:mc-test-power}}
\resizebox{\textwidth}{!}{\setlength{\tabcolsep}{4pt}
\begin{tabular}{rlc cccccccc}
\toprule
$T$ & Design & $\delta$ & Bound & CVAR test & Robust & PR & EG & Johansen & ECR & Wald\\
\midrule
200 & Triangular, $k=1$ & 0.0 & 0.724 & 0.664 & 0.523 & 0.408 & 0.229 & 0.108 & 0.257 & 0.214\\
200 & Triangular, $k=1$ & 0.6 & 0.932 & 0.112 & 0.525 & 0.267 & 0.169 & 0.196 & 0.317 & 0.295\\
200 & Triangular, $k=3$ & 0.0 & 0.769 & 0.561 & 0.416 & 0.166 & 0.160 & 0.085 & 0.160 & 0.114\\
200 & Triangular, $k=3$ & 0.6 & 0.922 & 0.145 & 0.160 & 0.141 & 0.121 & 0.102 & 0.218 & 0.202\\
200 & CVAR, $K=3$ & 0.0 &  & 0.181 & 0.115 & 0.152 & 0.155 & 0.083 & 0.107 & 0.083\\
200 & CVAR, $K=3$ & 0.6 &  & 0.154 & 0.133 & 0.068 & 0.036 & 0.084 & 0.146 & 0.129\\
200 & CVAR, $K=6$ & 0.0 &  & 0.248 & 0.131 & 0.125 & 0.123 & 0.037 & 0.121 & 0.088\\
200 & CVAR, $K=6$ & 0.6 &  & 0.130 & 0.107 & 0.080 & 0.060 & 0.060 & 0.111 & 0.106\\
400 & Triangular, $k=1$ & 0.0 & 0.714 & 0.653 & 0.494 & 0.396 & 0.232 & 0.115 & 0.230 & 0.212\\
400 & Triangular, $k=1$ & 0.6 & 0.948 & 0.108 & 0.547 & 0.400 & 0.221 & 0.253 & 0.382 & 0.370\\
400 & Triangular, $k=3$ & 0.0 & 0.624 & 0.551 & 0.380 & 0.182 & 0.160 & 0.068 & 0.213 & 0.124\\
400 & Triangular, $k=3$ & 0.6 & 0.922 & 0.103 & 0.184 & 0.122 & 0.084 & 0.095 & 0.217 & 0.206\\
400 & CVAR, $K=3$ & 0.0 &  & 0.233 & 0.131 & 0.177 & 0.198 & 0.118 & 0.198 & 0.144\\
400 & CVAR, $K=3$ & 0.6 &  & 0.196 & 0.145 & 0.084 & 0.038 & 0.096 & 0.151 & 0.188\\
400 & CVAR, $K=6$ & 0.0 &  & 0.324 & 0.232 & 0.091 & 0.125 & 0.060 & 0.133 & 0.094\\
400 & CVAR, $K=6$ & 0.6 &  & 0.117 & 0.089 & 0.071 & 0.045 & 0.052 & 0.110 & 0.156\\
\bottomrule
\end{tabular}}
\end{table}


==> exhibits/table13.tex <==
\begin{table}[H]
\centering\small
\caption{Order of the autoregression in the sieve bootstrap, CVAR design. Rejection rates at 5 percent under the null ($g=0$) and at $\rho=1-10/T$ ($g=10$), for the asymptotic critical value and for the bootstrap with $p$ lags; $\bar c=-7$. The rule $p_T=\lceil16(T/200)^{1/3}\rceil$ gives 16 lags at $T=200$ and 21 at $T=400$. 1000 replications, 199 bootstrap draws; dashes mark orders not run.\label{tab:mc-test-lags}}
\resizebox{\textwidth}{!}{\setlength{\tabcolsep}{4pt}
\begin{tabular}{rrc c cccc cccc}
\toprule
 & & & & \multicolumn{4}{c}{Size, bootstrap with $p$ lags} & \multicolumn{4}{c}{Power, bootstrap with $p$ lags}\\
\cmidrule(lr){5-8}\cmidrule(lr){9-12}
$T$ & $K$ & $\delta$ & Asymptotic & 12 & 16 & 20 & 24 & 12 & 16 & 20 & 24\\
\midrule
200 & 3 & 0.0 & 0.083 & 0.056 & -- & -- & 0.033 & 0.237 & -- & -- & 0.119\\
200 & 3 & 0.6 & 0.093 & 0.070 & -- & -- & 0.041 & 0.222 & -- & -- & 0.131\\
200 & 6 & 0.0 & 0.115 & 0.076 & -- & -- & 0.039 & 0.241 & -- & -- & 0.134\\
200 & 6 & 0.6 & 0.102 & 0.066 & -- & -- & 0.034 & 0.128 & -- & -- & 0.079\\
400 & 3 & 0.0 & 0.099 & 0.083 & 0.056 & 0.059 & 0.048 & 0.275 & 0.261 & 0.251 & 0.191\\
400 & 3 & 0.6 & 0.098 & 0.081 & 0.054 & 0.044 & 0.055 & 0.319 & 0.281 & 0.235 & 0.226\\
400 & 6 & 0.0 & 0.087 & 0.068 & 0.068 & 0.059 & 0.049 & 0.406 & 0.358 & 0.306 & 0.267\\
400 & 6 & 0.6 & 0.069 & 0.058 & 0.050 & 0.047 & 0.041 & 0.144 & 0.156 & 0.132 & 0.103\\
\bottomrule
\end{tabular}}
\end{table}


==> exhibits/table14.tex <==
\begin{table}[H]
\centering\small
\caption{Policies that react to the treated unit. Size at 5 percent ($g=0$) and size-adjusted power at $\rho=1-10/T$ ($g=10$) of the CVAR test, of its bootstrap version (autoregression of order $p_T=\lceil16(T/200)^{1/3}\rceil$), and of the augmented statistic with 4 and 12 lags of $\Delta Y^1_t$. Feedback from own change: the policy reacts to the twelve-month change of the treated unit; feedback from own level: to the level of its specific component. 1000 replications, 199 bootstrap draws.\label{tab:mc-test-feedback}}
\resizebox{\textwidth}{!}{\setlength{\tabcolsep}{4pt}
\begin{tabular}{rl cccc ccc}
\toprule
 & & \multicolumn{4}{c}{Size} & \multicolumn{3}{c}{Size-adjusted power}\\
\cmidrule(lr){3-6}\cmidrule(lr){7-9}
$T$ & Design & CVAR test & Bootstrap & Augm. 4 & Augm. 12 & CVAR test & Augm. 4 & Augm. 12\\
\midrule
200 & No feedback & 0.076 & 0.047 & 0.054 & 0.090 & 0.234 & 0.158 & 0.102\\
200 & Serially correlated cycle & 0.035 & 0.020 & 0.101 & 0.151 & 0.446 & 0.323 & 0.147\\
200 & Feedback from own change & 0.078 & 0.053 & 0.053 & 0.076 & 0.278 & 0.180 & 0.099\\
200 & Feedback and serial correlation & 0.027 & 0.022 & 0.088 & 0.131 & 0.437 & 0.268 & 0.100\\
200 & Feedback from own level & 0.086 & 0.066 & 0.055 & 0.086 & 0.216 & 0.167 & 0.113\\
400 & No feedback & 0.063 & 0.051 & 0.035 & 0.052 & 0.316 & 0.255 & 0.160\\
400 & Serially correlated cycle & 0.031 & 0.025 & 0.086 & 0.108 & 0.537 & 0.435 & 0.298\\
400 & Feedback from own change & 0.066 & 0.052 & 0.031 & 0.034 & 0.381 & 0.278 & 0.185\\
400 & Feedback and serial correlation & 0.028 & 0.031 & 0.070 & 0.098 & 0.583 & 0.493 & 0.235\\
400 & Feedback from own level & 0.065 & 0.050 & 0.028 & 0.047 & 0.327 & 0.235 & 0.142\\
\bottomrule
\end{tabular}}
\end{table}


==> exhibits/table15.tex <==
\begin{table}[H]
\centering\small
\caption{Conditional and adaptive tests, $T=200$. Size-adjusted power at $\rho=1-10/T$ for the bound, the CVAR test, the conditional tests CPO$_C$ and CPO$_K$, the adaptive test, and the error-correction tests; size at 5 percent of the CVAR test and of the adaptive test with critical values from the null with uncorrelated innovations of the same design. $\bar c=-7$, as in Section \ref{sec:test}. 2000 replications.\label{tab:supp-cpo}}
\resizebox{\textwidth}{!}{\setlength{\tabcolsep}{4pt}
\begin{tabular}{lc ccccccc cc}
\toprule
 & & \multicolumn{7}{c}{Size-adjusted power} & \multicolumn{2}{c}{Size}\\
\cmidrule(lr){3-9}\cmidrule(lr){10-11}
Design & $\delta$ & Bound & CVAR test & CPO$_C$ & CPO$_K$ & Adaptive & ECR & Wald & CVAR test & Adaptive\\
\midrule
Triangular, $k=3$ & 0.0 & 0.736 & 0.600 & 0.015 & 0.015 & 0.439 & 0.160 & 0.092 & 0.050 & 0.050\\
Triangular, $k=3$ & 0.3 & 0.791 & 0.368 & 0.019 & 0.018 & 0.238 & 0.191 & 0.140 & 0.054 & 0.062\\
Triangular, $k=3$ & 0.6 & 0.919 & 0.100 & 0.197 & 0.204 & 0.150 & 0.174 & 0.174 & 0.056 & 0.052\\
Triangular, $k=3$ & 0.9 & 1.000 & 0.011 & 0.941 & 0.940 & 0.907 & 0.447 & 0.777 & 0.050 & 0.062\\
Triangular, $k=1$ & 0.0 & 0.689 & 0.603 & 0.076 & 0.086 & 0.420 & 0.199 & 0.152 & 0.050 & 0.050\\
Triangular, $k=1$ & 0.6 & 0.931 & 0.117 & 0.638 & 0.651 & 0.542 & 0.308 & 0.342 & 0.044 & 0.046\\
CVAR, $K=3$ & 0.0 &  & 0.228 & 0.026 & 0.029 & 0.146 & 0.143 & 0.106 & 0.050 & 0.050\\
CVAR, $K=3$ & 0.6 &  & 0.211 & 0.017 & 0.019 & 0.145 & 0.131 & 0.118 & 0.072 & 0.058\\
CVAR, $K=6$ & 0.0 &  & 0.261 & 0.021 & 0.019 & 0.153 & 0.112 & 0.073 & 0.050 & 0.050\\
CVAR, $K=6$ & 0.6 &  & 0.123 & 0.049 & 0.049 & 0.098 & 0.100 & 0.082 & 0.050 & 0.037\\
\bottomrule
\end{tabular}}
\end{table}


==> xr-main.tex <==
% Labels of main.tex, frozen by make_arxiv.py; do not edit.
\newlabel{sec:intro}{{1}{2}{Introduction}{}{}}
\newlabel{tab:methods}{{1}{6}{What each approach allows}{}{}}
\newlabel{sec:causal}{{2}{6}{Causal framework}{}{}}
\newlabel{eq:po}{{1}{7}{Causal framework}{}{}}
\newlabel{eq:effectpath}{{2}{7}{Causal framework}{}{}}
\newlabel{def:ice}{{1}{8}{Impulse causal effect}{}{}}
\newlabel{eq:ice}{{3}{8}{Impulse causal effect}{}{}}
\newlabel{def:regime}{{2}{8}{Regime effect}{}{}}
\newlabel{eq:regime}{{4}{8}{Regime effect}{}{}}
\newlabel{eq:innovation}{{5}{8}{Causal framework}{}{}}
\newlabel{def:surprise}{{3}{9}{Effect of a policy surprise}{}{}}
\newlabel{eq:estimand}{{6}{9}{Effect of a policy surprise}{}{}}
\newlabel{sec:assumptions}{{3}{9}{Assumptions}{}{}}
\newlabel{assu:A1}{{1}{9}{No anticipation, no interference and untreated controls}{}{}}
\newlabel{assu:A2}{{2}{10}{Common trends}{}{}}
\newlabel{eq:factors}{{7}{10}{Common trends}{}{}}
\newlabel{eq:cycle0}{{8}{10}{Assumptions}{}{}}
\newlabel{assu:A3}{{3}{11}{Additive dynamic effects}{}{}}
\newlabel{eq:decomp}{{9}{11}{Assumptions}{}{}}
\newlabel{assu:A3b}{{3$'$}{11}{Linear policy response}{}{}}
\newlabel{eq:pathbias}{{10}{11}{Assumptions}{}{}}
\newlabel{eq:cycle}{{11}{12}{Assumptions}{}{}}
\newlabel{assu:A4}{{4}{12}{Exogeneity with respect to the counterfactual cycle}{}{}}
\newlabel{assu:A5}{{5}{12}{Stationarity and moments}{}{}}
\newlabel{sec:theorems}{{4}{12}{Theorems}{}{}}
\newlabel{sec:var}{{4.1}{12}{What a VAR without controls estimates}{}{}}
\newlabel{thm:var}{{1}{12}{What a VAR without controls identifies}{}{}}
\newlabel{eq:bias}{{12}{12}{What a VAR without controls identifies}{}{}}
\newlabel{sec:cvar}{{4.2}{13}{The CVAR}{}{}}
\newlabel{thm:cycle}{{2}{13}{What the CVAR identifies}{}{}}
\newlabel{eq:cyclebias}{{13}{13}{What the CVAR identifies}{}{}}
\newlabel{thm:ident}{{3}{14}{Identification}{}{}}
\newlabel{thm:direct}{{4}{15}{Impulse causal effects and regime effects}{}{}}
\newlabel{sec:bounds}{{4.3}{15}{Bounds}{}{}}
\newlabel{prop:placebo}{{1}{16}{Response of the controls}{}{}}
\newlabel{assu:A4b}{{4$'$}{16}{Bounded bias specific to the treated unit}{}{}}
\newlabel{prop:bounds}{{2}{17}{Bounds}{}{}}
\newlabel{sec:estimation}{{4.4}{17}{Estimation and inference}{}{}}
\newlabel{eq:dols}{{14}{18}{Estimation and inference}{}{}}
\newlabel{thm:est}{{5}{19}{Estimated weights}{}{}}
\newlabel{eq:firststep}{{15}{19}{Estimated weights}{}{}}
\newlabel{thm:joint}{{6}{21}{Estimated weights, long autoregressions and the bootstrap}{}{}}
\newlabel{sec:test}{{5}{23}{Testing the design}{}{}}
\newlabel{eq:testmodel}{{16}{23}{Testing the design}{}{}}
\newlabel{eq:PT}{{17}{23}{Testing the design}{}{}}
\newlabel{thm:po}{{7}{24}{Asymptotic equivalence with the known-weights test}{}{}}
\newlabel{sec:ext}{{6}{25}{A treated unit with a trend of its own}{}{}}
\newlabel{assu:A2d}{{6}{26}{Common trends and a trend of the treated unit}{}{}}
\newlabel{eq:cumcycle}{{18}{26}{A treated unit with a trend of its own}{}{}}
\newlabel{assu:A4d}{{7}{26}{Exogeneity with respect to the changes of the counterfactual cycle}{}{}}
\newlabel{thm:diff}{{8}{27}{Response of the cumulated cycle}{}{}}
\newlabel{prop:wchanges}{{3}{28}{Weights estimated in changes}{}{}}
\newlabel{sec:alaska}{{7}{29}{The Alaska Permanent Fund Dividend}{}{}}
\newlabel{tab:ak-weights}{{2}{32}{Weights on the donor states, reproduction of the common movement and tests of the design}{}{}}
\newlabel{fig:ak-main}{{1}{33}{Alaska Permanent Fund Dividend: cumulated response to a dividend larger by \$1,000 per person. CVAR with 68 and 90 percent bands, VAR without controls with its 90 percent band, and response of the weighted controls in the VAR with Alaska and the weighted controls. Rates in percentage points, employment in percent. Monthly, January 1976 (payroll series January 1990) to December 2019}{}{}}
\newlabel{tab:ak-main}{{3}{34}{Response to a dividend of \$1,000 per person}{}{}}
\newlabel{sec:ebsum}{{8}{35}{Extended unemployment benefits}{}{}}
\newlabel{sec:lcfssum}{{9}{35}{The Low Carbon Fuel Standard}{}{}}
\newlabel{sec:conclusions}{{10}{36}{Conclusions}{}{}}
\newlabel{sec:proofs-main}{{A}{38}{Proofs of the main results}{}{}}
\newlabel{lem:dl}{{1}{38}{Responses of distributed lags}{}{}}
\newlabel{eq:Sdecomp}{{19}{45}{Proofs for Section \ref {sec:test}}{}{}}
\newlabel{lem:fclt}{{2}{45}{}{}{}}
\newlabel{lem:orders}{{3}{46}{}{}{}}
\newlabel{lem:lrv}{{4}{47}{}{}{}}
\newlabel{sec:data}{{B}{50}{Data sources}{}{}}
\newlabel{tab:data}{{4}{50}{Data sources}{}{}}

